Free precategories as presheaf categories

Precategories generalize both the notions of strict $n$-category and sesquicategory: their definition is essentially the same as the one of strict $n$-categories, excepting that we do not require the various interchange laws to hold. Those have been proposed as a framework in which one can express semi-strict definitions of weak higher categories: in dimension 3, Gray categories are an instance of them and have been shown to be equivalent to tricategories, and definitions of semi-strict tetracategories have been proposed, and used as the basis of proof assistants such as Globular. In this article, we are mostly interested in free precategories. Those can be presented by generators and relations, using an appropriate variation on the notion of polygraph (aka computad), and earlier works have shown that the theory of rewriting can be generalized to this setting, enjoying most of the fundamental constructions and properties which can be found in the traditional theory, contrarily to polygraphs for strict categories. We further study here why this is the case, by providing several results which show that precategories and their associated polygraphs bear properties which ensure that we have a good syntax for those. In particular, we show that the category of polygraphs for precategories form a presheaf category.

==> Makefile <==
ARXIV_OUT=arxiv_temp
ARXIV_REMOVED=temp.tex NOTES.md README.md prog temp.tex placard.tex

all: article satex

article: satex
	rubber -d article

satex:
	$(MAKE) -C satex

ci:
	git ci . -m "Worked on precategories."
	git push

clean:
	rm -f *.aux *.bbl *.bcf *.blg *.log *.out *.rubbercache *.run.xml *.toc *.pdf

upload: article
	scp article.pdf lix:.webdir/docs/mimram_free_precat.pdf

arxiv:
# to be executed in the archive generated by arxiv_archive in order to get the arxiv version
	rubber -d article
	cp article.pdf ../article-arxiv.pdf
#	echo "SF: pour mettre à jour le pdf sur le site, faire 'make update_site'."

arxiv_archive: SHELL:=/bin/bash
arxiv_archive:
	rm -rf ${ARXIV_OUT}
	mkdir ${ARXIV_OUT}
	git archive --format=tar HEAD . | (cd ${ARXIV_OUT}; tar xf -)
	make -j4 -C satex satix
	(cd ${ARXIV_OUT};\
	make -j4 -C satex satix;\
	rm -r ${ARXIV_REMOVED};\
	cp ../article.bbl article.bbl;\
	sed -i $$'/%%% ARXIV-PLACEHOLDER/{z;rarxiv.tex\n}' macros.sty;\
	tar cvzf arxiv.tar.gz *;\
	cp -i arxiv.tar.gz ../arxiv.tar.gz)

.PHONY: satex


==> arxiv.tex <==
% to be added in the arxiv version (no other pdf allowed, figs must be recomputed)
\usepackage{xkeyval}
\makeatletter
\define@key{satex}{scale}{\def\satex@scale{#1}}
\newcommand{\defsatexfig}[2]{\expandafter\newcommand\csname satexfigure#1\endcsname{#2}}
\renewcommand{\satex}[2][]{%
  \expandafter\let\csname satexfigure0\endcsname\undefined
  \def\satex@scale{0.9}\setkeys{satex}{#1}%
  \IfFileExists{satex/#2.satix}{\input{satex/#2.satix}}{\@latex@error{No
      file #2.satix}.}%
  \vcenter{%
    \hbox{\scalebox{\satex@scale}{%
        \csname satexfigure0\endcsname
      }}}}
\renewcommand{\satexnoscale}{\satex}
\makeatother
